Reducing Computational Complexity of Tensor Contractions via Tensor-Train Networks

There is a significant expansion in both volume and range of applications along with the concomitant increase in the variety of data sources. These ever-expanding trends have highlighted the necessity for more versatile analysis tools that offer greater opportunities for algorithmic developments and computationally faster operations than the standard flat-view matrix approach. Tensors, or multi-way arrays, provide such an algebraic framework which is naturally suited to data of such large volume, diversity, and veracity. Indeed, the associated tensor decompositions have demonstrated their potential in breaking the Curse of Dimensionality associated with traditional matrix methods, where a necessary exponential increase in data volume leads to adverse or even intractable consequences on computational complexity. A key tool underpinning multi-linear manipulation of tensors and tensor networks is the standard Tensor Contraction Product (TCP). However, depending on the dimensionality of the underlying tensors, the TCP also comes at the price of high computational complexity in tensor manipulation. In this work, we resort to diagrammatic tensor network manipulation to calculate such products in an efficient and computationally tractable manner, by making use of Tensor Train decomposition (TTD). This has rendered the underlying concepts easy to perceive, thereby enhancing intuition of the associated underlying operations, while preserving mathematical rigour. In addition to bypassing the cumbersome mathematical multi-linear expressions, the proposed Tensor Train Contraction Product model is shown to accelerate significantly the underlying computational operations, as it is independent of tensor order and linear in the tensor dimension, as opposed to performing the full computations through the standard approach (exponential in tensor order).

==> 04-tikz/contraction-all-but-N.tex <==
% !TEX root = ../main.tex
% cSpell:disable
% cSpell:ignoreRegExp ^[\s]*%.*
% cSpell:ignoreRegExp \\[0-9a-zA-Z]*
% cSpell:ignoreRegExp .*\\usepackage.*
% cSpell:ignoreRegExp .*\\cite\{[\w:\-,\s]*\}
% cSpell:ignoreRegExp .*\\c?ref\{[\w:\-]*\}
% cSpell:ignoreRegExp .*\\(begin|end){.*}.*


%----- Font sizes
\newcommand{\fontLeafs}[1]{\scalebox{5.5}{#1}} % this is for leafs labels
\newcommand{\fontTNodes}[1]{\scalebox{7}{#1}} % this is for TN cores labels
\newcommand{\fontEq}[1]{\scalebox{10}{#1}} % this is for equation signs

%----- Sizes and Offsets
\newcommand{\localLeafSize}{5cm}         % size of leafs of just tensor
\newcommand{\xShift}{36cm}           % horizontal shift for the starting points
\newcommand{\yShift}{15cm}           % vertical shift for different parts
\newcommand{\yShiftLeaf}{3cm}       % vertical shift for the leaf from the main line (center of core tensor)

\newdimen\xRefOne
\newdimen\xRefTwo
\newdimen\xRefThree
\newdimen\xRefFour
\newdimen\xRefFive
\newdimen\xRefSix
\newdimen\xRefSeven
\newdimen\xRefEight
\newdimen\xRefNine
\newdimen\xRefTen
\newdimen\xRefEleven
\newdimen\yLevel

\newcommand{\setAllRefPoints}{
    % Reference point list
    % name | place | node | point of this node
    % reference points from ref1 through ref10 lay on the main horizontal line for the
    % current level and equally spaced between TWO and THREE
    \coordinate (TWO) at ($(ONE) + (\xShift/3,0)$);
    \coordinate (THREE) at ($(TWO) + (\xShift,0)$);
    \coordinate (FOUR) at ($(THREE) + (\xShift/3,0)$);

    \setCoordinateX{$(TWO)!1/11!(THREE)$}{\xRefOne}
    \setCoordinateX{$(TWO)!2/11!(THREE)$}{\xRefTwo}
    \setCoordinateX{$(TWO)!3/11!(THREE)$}{\xRefThree}
    \setCoordinateX{$(TWO)!4/11!(THREE)$}{\xRefFour}
    \setCoordinateX{$(TWO)!5/11!(THREE)$}{\xRefFive}
    \setCoordinateX{$(TWO)!6/11!(THREE)$}{\xRefSix}
    \setCoordinateX{$(TWO)!7/11!(THREE)$}{\xRefSeven}
    \setCoordinateX{$(TWO)!8/11!(THREE)$}{\xRefEight}
    \setCoordinateX{$(TWO)!9/11!(THREE)$}{\xRefNine}
    \setCoordinateX{$(TWO)!10/11!(THREE)$}{\xRefTen}

    \setCoordinateY{TWO.center}{\yLevel}
    \coordinate (ref1) at (\xRefOne,\yLevel);
    \coordinate (ref2) at (\xRefTwo,\yLevel);
    \coordinate (ref3) at (\xRefThree,\yLevel);
    \coordinate (ref4) at (\xRefFour,\yLevel);
    \coordinate (ref5) at (\xRefFive,\yLevel);
    \coordinate (ref6) at (\xRefSix,\yLevel);
    \coordinate (ref7) at (\xRefSeven,\yLevel);
    \coordinate (ref8) at (\xRefEight,\yLevel);
    \coordinate (ref9) at (\xRefNine,\yLevel);
    \coordinate (ref10) at (\xRefTen,\yLevel);
    \coordinate (ref11) at (\xRefEleven,\yLevel);
}
\newcommand{\drawAllRefPoints}{
    %% this is for checking where the reference points are
    \draw (ref1) -- ($(ref1) + (0,\yShiftLeaf)$);
    \draw (ref2) -- ($(ref2) + (0,\yShiftLeaf)$);
    \draw (ref3) -- ($(ref3) + (0,\yShiftLeaf)$);
    \draw (ref4) -- ($(ref4) + (0,\yShiftLeaf)$);
    \draw (ref5) -- ($(ref5) + (0,\yShiftLeaf)$);
    \draw (ref6) -- ($(ref6) + (0,\yShiftLeaf)$);
    \draw (ref7) -- ($(ref7) + (0,\yShiftLeaf)$);
    \draw (ref8) -- ($(ref8) + (0,\yShiftLeaf)$);
    \draw (ref9) -- ($(ref9) + (0,\yShiftLeaf)$);
    \draw (ref10) -- ($(ref10) + (0,\yShiftLeaf)$);
    \draw (ref11) -- ($(ref11) + (0,\yShiftLeaf)$);
    \draw[red] (core.center) -- ($(ref1) + (0,\yShiftLeaf)$) -- ($(ref3) + (0,\yShiftLeaf)$) -- (ref4) -- (ref7) -- ($(ref8) + (0,\yShiftLeaf)$) -- ($(ref10) + (0,\yShiftLeaf)$);
}
\newcommand{\drawEqSign}{
    \coordinate (temp1) at ($(ref4)!1/2!(ref7)$);
    \coordinate (temp2) at ($(temp1) + (0,-\yShift)$);
    \node[no sep,anchor=center,rotate=90] (l) at ($(temp1)!1/2!(temp2)$) {\fontEq{$\Leftrightarrow$}};
}


\begin{tikzpicture}
\setTNsTikzset[leaf size=\localLeafSize]

%%====== First row from the top part
\coordinate (ONE) at (0,0);
\setAllRefPoints

\draw[round corners]
    (TWO) --
    ($(ref1)  + (0,\yShiftLeaf)$) --
    ($(ref10) + (0,\yShiftLeaf)$) --
    (THREE);
\draw[round corners]
    (TWO) --
    ($(ref1)  + (0,-\yShiftLeaf)$) --
    ($(ref10) + (0,-\yShiftLeaf)$) --
    (THREE);

\tnode[name=X, start at=TWO]{}{\fontTNodes{$\ten{X}$}};
\tnode[name=Y, start at=THREE]{}{\fontTNodes{$\ten{Y}$}};
\tnLeafEE[start at=Y, label=\fontLeafs{$J_3$}]{}{}{}{2*\localLeafSize};
\tnLeafWW[start at=X, label=\fontLeafs{$I_3$}]{}{}{}{2*\localLeafSize};

\coordinate (tmp) at ($(TWO)!1/2!(THREE) + (0,\yShiftLeaf)$);
\tnLeafCC[name=I2, start at=tmp, label=\fontLeafs{$I_1 = J_1$}]{}{}{}{0};

\coordinate (tmp) at ($(TWO)!1/2!(THREE) + (0,-\yShiftLeaf)$);
\tnLeafCC[name=I3, start at=tmp, label=\fontLeafs{$I_2 = J_2$}]{}{}{}{0};
\drawEqSign;



%%====== Second row from the top part
\coordinate (ONE) at ($(ONE) - (0,\yShift)$);
\setAllRefPoints

\draw[round corners]
    (TWO) --
    ($(ref1) + (0,\yShiftLeaf)$) --
    ($(ref3) + (0,\yShiftLeaf)$) --
    (ref4) --
    (ref7) --
    ($(ref8)  + (0,\yShiftLeaf)$) --
    ($(ref10) + (0,\yShiftLeaf)$) --
    (THREE);
\draw[round corners]
    (TWO) --
    ($(ref1) + (0,-\yShiftLeaf)$) --
    ($(ref3) + (0,-\yShiftLeaf)$) --
    (ref4) --
    (ref7) --
    ($(ref8)  + (0,-\yShiftLeaf)$) --
    ($(ref10) + (0,-\yShiftLeaf)$) --
    (THREE);

\tnode[name=X, start at=TWO]{}{\fontTNodes{$\ten{X}$}};
\tnode[name=Y, start at=THREE]{}{\fontTNodes{$\ten{Y}$}};
\tnLeafEE[start at=Y, label=\fontLeafs{$J_3$}]{}{}{}{2*\localLeafSize};
\tnLeafWW[start at=X, label=\fontLeafs{$I_3$}]{}{}{}{2*\localLeafSize};

\node[unfolding] (unfolding) at (ref4) {}; \node[anchor=east] () at (unfolding.west) {\fontLeafs{$3$}};
\coordinate (tmp) at ($(TWO)!1/2!(ref4) + (0,\yShiftLeaf)$);
\tnLeafCC[name=R2, start at=tmp, label=\fontLeafs{$I_1$}]{}{}{}{0};
\coordinate (tmp) at ($(TWO)!1/2!(ref4) + (0,-\yShiftLeaf)$);
\tnLeafCC[name=R3, start at=tmp, label=\fontLeafs{$I_2$}]{}{}{}{0};


\coordinate (tmp) at ($(TWO)!1/2!(THREE)$);
\tnLeafCC[name=R2R3, start at=tmp, label=\fontLeafs{$I_1 I_2 = J_1 J_2$}]{}{}{}{};


\node[unfolding] (unfolding) at (ref7) {}; \node[anchor=west] () at (unfolding.east) {\fontLeafs{$3$}};
\coordinate (tmp) at ($(THREE)!1/2!(ref7) + (0,\yShiftLeaf)$);
\tnLeafCC[name=R2, start at=tmp, label=\fontLeafs{$J_1$}]{}{}{}{0};
\coordinate (tmp) at ($(THREE)!1/2!(ref7) + (0,-\yShiftLeaf)$);
\tnLeafCC[name=R3, start at=tmp, label=\fontLeafs{$J_2$}]{}{}{}{0};

\drawEqSign;




%%====== Third row from the top part
\coordinate (ONE) at ($(ONE) - (0,\yShift)$);
\setAllRefPoints

\draw[round corners]
    (TWO) --
    (THREE);

\mnode[name=X, start at=TWO]{}{\fontTNodes{$\unfold{X}{3}$}};
\mnode[name=Y, start at=THREE]{}{\fontTNodes{$\unfold{Y}{3}^T$}};
\tnLeafEE[start at=Y, label=\fontLeafs{$J_3$}]{}{}{}{2*\localLeafSize};
\tnLeafWW[start at=X, label=\fontLeafs{$I_3$}]{}{}{}{2*\localLeafSize};

\coordinate (tmp) at ($(TWO)!1/2!(THREE)$);
\tnLeafCC[name=R2R3, start at=tmp, label=\fontLeafs{$R_2R_3$}]{}{}{}{};

\end{tikzpicture}


==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************

